Beauty Beyond Words: Explainable Beauty Product Recommendations Using Ingredient-Based Product Attributes

Accurate attribute extraction is critical for beauty product recommendations and building trust with customers. This remains an open problem, as existing solutions are often unreliable and incomplete. We present a system to extract beauty-specific attributes using end-to-end supervised learning based on beauty product ingredients. A key insight to our system is a novel energy-based implicit model architecture. We show that this implicit model architecture offers significant benefits in terms of accuracy, explainability, robustness, and flexibility. Furthermore, our implicit model can be easily fine-tuned to incorporate additional attributes as they become available, making it more useful in real-world applications. We validate our model on a major e-commerce skincare product catalog dataset and demonstrate its effectiveness. Finally, we showcase how ingredient-based attribute extraction contributes to enhancing the explainability of beauty recommendations.

==> Sections/ToDo.tex <==
\section{TODO}

\begin{itemize}
    \item Clarification on BT-BERT performance (Page 5): The authors mention, We hypothesize that the robust performance of BT-BERT in such a low-resource regime can be attributed to the fact that it is an energy-based implicit model, as opposed to an explicit classifier. I do not fully agree with this point, because, based on Table 1, which shows the model performance for the explicit vs. implicit approach (BT-BERT), the explicit model performs quite well and is close to the implicit model (unlike the Fuzzy Search model).
\end{itemize}

==> Sections/problem.tex <==
\section{Customer Problem Statement}

Product discovery is one of the biggest problems in customer shopping journey on e-commerce sites.
Many factors contribute to this problem, such as non-personalized recommendations, but ultimately the root cause can be traced to inaccurate or incomplete information provided by sellers. 
Sometimes the benefits of products are intentionally exaggerated to mislead the customers, and other times the seller simply does not have the scientific expertise to accurately label the products.
This type of misinformation can have significant negative impact on customers' health and well-being, especially for beauty products that are directly applied to the skin.
% As a result, customers lose trust and shop on competing platforms.
In the short-term, our work will benefit both the customers and sellers by automatically extracting the attribute labels from product ingredients and title.
It will also help fostering customer trust over the long run.

% % 1) dont know what is product is right for them
% % 2) hard to find which one to choose, does they work? harmful for skin cand hair!
% Beauty customers often find it difficult narrowing down the right products they are looking for from billions of e-commerce platform.
% They often identify a beauty product's functionality by looking at product description provided by sellers.
% Often times, beauty products are often do not effect than they are claimed to work.
% Most critically, some of them can create harmful impact to customers' face and body, and this is especially true for skincare and haircare products. 
% % overexerted.... 
% % should I add an exmaple here? 
% Additionally, beauty customers replies on customer reviews to verify how products works on human objects. 
% Nevertheless, beauty products are very personalized. 
% A customer with oily skin may prefer skincare products with AHA/BHA ingredients to reduce sebum production; while AHA/BHA might be cause irritation for customer with sensitive skin, and even dry out customer with dry skin type. 
% Last but not the least, the information is not always listed on the product page. 
